Complexity and Avoidance

In this dissertation we examine the relationships between the several hierarchies, including the complexity, $\mathrm{LUA}$ (Linearly Universal Avoidance), and shift complexity hierarchies, with an eye towards quantitative bounds on growth rates therein. We show that for suitable $f$ and $p$, there are $q$ and $g$ such that $\mathrm{LUA}(q) \leq_\mathrm{s} \mathrm{COMPLEX}(f)$ and $\mathrm{COMPLEX}(g) \leq_\mathrm{s} \mathrm{LUA}(p)$, as well as quantify the growth rates of $q$ and $g$. In the opposite direction, we show that for certain sub-identical $f$ satisfying $\lim_{n \to \infty}{f(n)/n}=1$ there is a $q$ such that $\mathrm{COMPLEX}(f) \leq_\mathrm{w} \mathrm{LUA}(q)$, and for certain fast-growing $p$ there is a $g$ such that $\mathrm{LUA}(p) \leq_\mathrm{s} \mathrm{COMPLEX}(g)$, as well as quantify the growth rates of $q$ and $g$. Concerning shift complexity, explicit bounds are given on how slow-growing $q$ must be for any member of $\rm{LUA}(q)$ to compute $\delta$-shift complex sequences. Motivated by the complexity hierarchy, we generalize the notion of shift complexity to consider sequences $X$ satisfying $\operatorname{KP}(\tau) \geq f(|\tau|) - O(1)$ for all substrings $\tau$ of $X$ where $f$ is any order function. We show that for sufficiently slow-growing $f$, $f$-shift complex sequences can be uniformly computed by $g$-complex sequences, where $g$ grows slightly faster than $f$. The structure of the $\mathrm{LUA}$ hierarchy is examined using bushy tree forcing, with the main result being that for any order function $p$, there is a slow-growing order function $q$ such that $\mathrm{LUA}(p)$ and $\mathrm{LUA}(q)$ are weakly incomparable. Using this, we prove new results about the filter of the weak degrees of deep nonempty $\Pi^0_1$ classes and the connection between the shift complexity and $\mathrm{LUA}$ hierarchies.

==> ConvexityConcerns.tex <==
\begin{prop} \label{bounded jumps}
For any $\alpha>1$ and fast-growing $p$, there exists a fast-growing $\hat{p}$ such that $\hat{p} \domleq p$ and $\hat{p}(n+1)/\hat{p}(n) \leq \alpha$ for all $n \in \mathbb{N}$. Moreover, if $\sum_{n=0}^\infty{p(n)^{-1}}$ is recursive, then $\hat{p}$ can be chosen so that $\sum_{n=0}^\infty{\hat{p}(n)^{-1}}$ is recursive as well.
\end{prop}
\begin{proof}
Without loss of generality we may assume $\alpha$ is recursive. We define $\hat{p}$ recursively as follows:
\begin{align*}
\hat{p}(0) & \coloneq p(0), \\
\hat{p}(n+1) & \coloneq \min\{\alpha \hat{p}(n),p(n+1)\}.
\end{align*}
$\hat{p}$ is a recursive order function dominated by $p$, so it just remains to show that $\hat{p}$ is fast-growing and that if $\sum_{n=0}^\infty{p(n)^{-1}}$ is recursive then $\sum_{n=0}^\infty{\hat{p}(n)^{-1}}$ is recursive.

Define $I \coloneq \{ n \in \mathbb{N} \mid \hat{p}(n) = p(n)\}$. Note that $I$ is a recursive nonempty subset of $\mathbb{N}$. We consider two cases:
\begin{description}
\item[Case 1: $I$ finite.] Let $n_0 = \max I$. By the definition of $\hat{p}$ we then have $\hat{p}(n) = \alpha^{n-n_0}p(n_0)$ for all $n \geq n_0$. Thus,
\begin{equation*}
\sum_{n=0}^\infty{\hat{p}(n)^{-1}} = \sum_{n=0}^{n_0-1}{\hat{p}(n)^{-1}} + \frac{1}{p(n_0)} \sum_{n=n_0}^\infty{\frac{1}{\alpha^{n-n_0}}} = \sum_{n=0}^{n_0-1}{\hat{p}(n)^{-1}} + \frac{1}{p(n_0)}\cdot \frac{\alpha}{\alpha-1} < \infty.
\end{equation*}
Moreover, we quickly see that $\sum_{n=0}^\infty{\hat{p}(n)^{-1}}$ is a recursive real. 

\item[Case 2: $I$ infinite.] Let $\langle n_k \rangle_{k \in \mathbb{N}}$ be the strictly increasing enumeration of $I$. Then
\begin{equation*}
\sum_{n=0}^\infty{\hat{p}(n)^{-1}} = \sum_{k=0}^\infty{\left(1+\frac{1}{\alpha} + \frac{1}{\alpha^2} + \cdots + \frac{1}{\alpha^{n_{k+1}-n_k-1}}\right)\frac{1}{p(n_k)}} \leq \frac{\alpha}{\alpha - 1}\sum_{k=0}^\infty{\frac{1}{p(n_k)}} \leq \frac{\alpha}{\alpha-1}\sum_{n=0}^\infty{p(n)^{-1}} < \infty.
\end{equation*}
Now suppose $\sum_{n=0}^\infty{p(n)^{-1}}$ is a recursive real, so that there is a nondecreasing recursive sequence $\langle N_m\rangle_{m \in \mathbb{N}}$ such that $\sum_{n=N_m}^\infty{p(n)^{-1}} \leq 2^{-m}$ for all $m \in \mathbb{N}$. Let $j$ be minimal such that $\frac{\alpha}{\alpha - 1} \leq 2^j$. We now define a recursive sequence $\langle k_m \rangle_{m \in \mathbb{N}}$ by setting $k_m$ to be the least $k$ such that $N_{m+j} \leq n_k$. Then
\begin{equation*}
\sum_{n=n_{k_m}}^\infty{\hat{p}(n)^{-1}} = \sum_{k=k_m}^\infty{\left(1+\frac{1}{\alpha} + \frac{1}{\alpha^2} + \cdots + \frac{1}{\alpha^{n_{k+1}-n_k-1}}\right)\frac{1}{p(n_k)}} \leq \frac{\alpha}{\alpha-1}\sum_{k=k_m}^\infty{\frac{1}{p(n_k)}} \leq \frac{\alpha}{\alpha-1}\sum_{n=n_{k_m}}^\infty{p(n)^{-1}} \leq \frac{\alpha}{\alpha-1}\sum_{n=N_{m+j}}^\infty{p(n)^{-1}} \leq \frac{\alpha}{\alpha-1} \frac{1}{2^{m+j}} \leq \frac{1}{2^m}.
\end{equation*}
It follows that $\sum_{n=0}^\infty{\hat{p}(n)^{-1}}$ is recursive.
\end{description}
\end{proof}

\begin{cor}
For any $\epsilon > 0$ and any fast-growing order function $p$ such that $\sum_{n=0}^\infty{p(n)^{-1}}$ is a recursive real there is a sub-identical order function $f$ such that $f(n+1)-f(n) \leq 1+\epsilon$ for all $n \in \mathbb{N}$ and $\ldnr(p) \strongleq \complex(f)$.
\end{cor}
\begin{proof}
Fix $\alpha > 1$ such that $1+4\log_2 \alpha \leq \epsilon$. By \cref{bounded jumps} we may assume without loss of generality that $p(n+1) \leq \alpha p(n)$ for all $n \in \mathbb{N}$. By \cref{}, if $\tilde{p}$ is a fast-growing order function such that $\lim_{n\to\infty}{\frac{p(n)}{\tilde{p}(n+3)}}=\infty$, then with $f$ defined by $f(n) \coloneq \log_2 \tilde{p}(p^{-1}(2^{n+2}-1))$ for $n \in \mathbb{N}$ we have $\ldnr(p) \strongleq \complex(f)$. 

The proof of \cref{} shows that we may take $\tilde{p}$ to be of the form $\tilde{p}(n) = 2^{-k(n-3)} p(n-3)$ for some order function $k\colon \mathbb{N} \to \mathbb{N}$, so that
\begin{equation*}
\lim_{n \to \infty}{\frac{p(n)}{\tilde{p}(n+3)}} = \lim_{n\to\infty}{\frac{p(n)}{2^{-k(n)}p(n)}} = \lim_{n \to \infty}{2^{k(n)}} = \infty.
\end{equation*}
Then for almost every $n \in \mathbb{N}$ we have
\begin{align*}
f(n+1)-f(n) & = \log_2 \tilde{p}(p^{-1}(2^{n+3})-1) - \log_2 \tilde{p}(p^{-1}(2^{n+2})-1) \\
& = \log_2\left( \frac{\tilde{p}(p^{-1}(2^{n+3})-1)}{\log_2 \tilde{p}(p^{-1}(2^{n+2})-1)}\right) \\
& = \log_2\left( \frac{2^{k(p^{-1}(2^{n+2})-4)} p(p^{-1}(2^{n+3})-4)}{2^{k(p^{-1}(2^{n+2})-4)} p(p^{-1}(2^{n+2})-4)}\right) \\
& \leq \log_2\left( \frac{p(p^{-1}(2^{n+3})-4)}{p(p^{-1}(2^{n+2})-4)}\right) \\
& \leq \log_2\left( \frac{2^{n+3}}{2^{n+2}/\alpha^4} \right) \\
& = 1 + 4\log_2 \alpha \\
& \leq 1+\epsilon.
\end{align*}
\end{proof}
